Exact Analytical Solution of the Flory-Huggins Model and Extensions to Multicomponent Systems

The Flory-Huggins theory describes the phase separation of solutions containing polymers. Although it finds widespread application from polymer physics to materials science to biology, the concentrations that coexist in separate phases at equilibrium have not been determined analytically, and numerical techniques are required that restrict the theory's ease of application. In this work, we derive an implicit analytical solution to the Flory-Huggins theory of one polymer in a solvent by applying a procedure that we call the implicit substitution method. While the solutions are implicit and in the form of composite variables, they can be mapped explicitly to a phase diagram in composition space. We apply the same formalism to multicomponent polymeric systems, where we find analytical solutions for polydisperse mixtures of polymers of one type. Finally, while complete analytical solutions are not possible for arbitrary mixtures, we propose computationally efficient strategies to map out coexistence curves for systems with many components of different polymer types.

==> main__Pedro_de_Souza_s_conflicted_copy_2024-03-29_.tex <==
% \documentclass[reprint,
% %preprint,
% superscriptaddress,
% %groupedaddress,
% %unsortedaddress,
% %runinaddress,
% %frontmatterverbose, 
% %preprint,
% %showpacs,preprintnumbers,
% %nofootinbib,
% %nobibnotes,
% %bibnotes,
% amsmath,amssymb,
% %aps,
% %prl,
% %pra,
% %prb,
% %rmp,
% %prstab,
% %prstper,
% %floatfix,
% ]{revtex4-1}

% \usepackage{xcolor}
% \usepackage{graphicx}% Include figure files
% \usepackage{dcolumn}% Align table columns on decimal point
% \usepackage{bm}% bold math
% \usepackage[utf8]{inputenc}
% \usepackage{upgreek}
% \usepackage{appendix}
% %\usepackage{hyperref}% add hypertext capabilities
% %\usepackage[mathlines]{lineno}% Enable numbering of text and display math
% %\linenumbers\relax % Commence numbering lines

% %\usepackage[showframe,%Uncomment any one of the following lines to test 
% %%scale=0.7, marginratio={1:1, 2:3}, ignoreall,% default settings
% %%text={7in,10in},centering,
% %%margin=1.5in,
% %%total={6.5in,8.75in}, top=1.2in, left=0.9in, includefoot,
% %%height=10in,a5paper,hmargin={3cm,0.8in},
% %]{geometry}

% \begin{document}

% \title{Exact Analytical Solution of the Flory-Huggins Model and Extensions to Multicomponent Systems}



% \author{J. Pedro de Souza}
% \author{Howard A. Stone}
% %  \email{pdesouza@mit.edu}
% % \affiliation{Department of Chemical Engineering, Massachusetts Institute of Technology, Cambridge, MA, USA}

% \date{\today}

% \begin{abstract}

% The Flory-Huggins theory describes the phase separation of solutions containing polymers. Although it finds widespread application from polymer physics to materials science to biology, the coexisting concentrations in separate phases at equilibrium have not previously been solved analytically, and numerical techniques are required that restrict the theory's ease of application. In this work, we derive an implicit analytical solution to the Flory-Huggins theory of one polymer in a solvent by applying a procedure that we call the implicit substitution method. While the solutions are implicit and in the form of composite variables, they can be explicitly mapped to a phase diagram in composition space. We apply the same formalism to multicomponent polymeric systems. There, we find analytical solutions for polydisperse mixtures of polymers of one type. Finally, while complete analytical solutions are not possible for arbitrary mixtures, we propose computationally efficient strategies to map out coexistence curves for systems with many components of different polymer types.

% \end{abstract}

% \maketitle

% %
% %Understanding ultra-concentrated electrolytes and ionic liquids (classical works, and recent advances*; theory vs experiments)
% %

% \section{Introduction}
% %Introduce phase separation and concentrated electrolytes

% Since its introduction in the early 1940s first by Huggins~\cite{huggins1941solutions} and then by Flory~\cite{flory1942thermodynamics}, the Flory-Huggins theory has become the most widespread model of polymer phase separation. Due to its simplicity in construction, it is able to capture the main trends in the polymer partitioning between phases with a minimal set of parameters.  The theory has been applied in numerous contexts from chemical processing ~\cite{cantow2013polymer, barton2018handbook} and also in the burgeoning field of biomolecular condensation~\cite{brangwynne2015polymer, berry2018physical, pappu2023phase}. While many corrections and modifications have been proposed to capture more detailed physical phenomena~\cite{overbeek1957phase, simha1969statistical, scheutjens1980statistical, tanaka1989theory, tanaka1994thermoreversible, semenov1998thermoreversible, ruzette2001simple, wang2008effects, wang201750th, wessen2021simple}, the original Flory-Huggins theory is the standard starting point for any analysis of materials that include polymeric components.

% From its physics based construction, the Flory-Huggins theory outputs a system of nonlinear constraints specifying thermodynamic equilibria that define the coexisting phase concentrations. While the equilibrium conditions can be solved numerically, up to this point, to our knowledge, no exact analytical solution has been found. Therefore, any evaluation of the theory or fitting of the theory to data requires numerical solutions, hampering the ease of use of the theory. In some regimes, analytical approximations can be applied~\cite{sanchez1984corresponding,tsenoglou2001slightly,scheinhardt2004stationary,qian2022analytical, van2023predicting}, but these approximations may involve complicated expressions and may not be uniformly valid, even for a single polymer-solvent combination.

% The technical challenge of describing coexisting phases is more apparent for multicomponent mixtures, even for mixtures of the same polymer type with different polymer lengths. In order to construct a phase diagram using direct numerical solution, it is necessary to discretize the compositional space, and solve nonlinear systems of equations at each point. As the number of polymer types, $M$, increases, the discretized space increases exponentially, with a power proportional to $M$, which corresponds to large number of discrete compositions, especially if fine resolution is desired. In many applications, such as in cellular biology, the number of polymer types can exceed tens of thousands. Such a brute force numerical approach may not be feasible to describe the breadth of coexisting concentrations over the full compositional space for $M>4$, never mind for $M>10^4$. 

% \begin{figure*}[t!]
% \centerline{\includegraphics[scale=0.75]{Fig1Draft.png}}
% \caption{Schematic of the systems under study, their corresponding variables, and the solution strategy employed in each case for (a) a single polymer-solvent solution (2) a polydisperse polymer-solvent solution, and (c) a solution containing multiple polymer types in solvent.}
% \end{figure*}

% Here, for the first time, we analytically derive an exact implicit solution to the Flory-Huggins theory of a one polymer-one solvent system using an implicit substitution method. The key idea is to solve each constraint for the Flory-Huggins $\chi$ parameter, and then substitute the value of $\chi$ into each equation so as to eliminate it from the system. We explore the solution's asymptotic behavior, referring back to the original applications of the theory by Flory.

% Next, we apply the implicit substitution method to multicomponent mixtures where the relative magnitude of the pair interactions are known. There, we discover an exact analytical solution for polydisperse polymer samples of the same type, and distill the phase diagram of these mixtures into two independent variables that fully specify the coexistence curves. Using this strategy, we can analytically describe the composition (molecular weight distribution and total polymer volume fraction) of the coexisting phases.

% For generalized mixtures, we use the implicit substitution method to simplify our nonlinear system of $M+1$ equations down to one nonlinear ``master'' equation with one unknown--- the solvent partitioning between the phases. While this reduction leads to great simplification of the equilibrium calculation, in the case of arbitrary mixtures, the master equation must be solved numerically. If desired, we can discretize the compositional space and construct a $\chi$ surface by solving just this one equation at each point---and we demonstrate this for a two polymer, one solvent mixture. To minimize the number of function evaluations, we propose a sampling method for the implicit function which obviates the need to discretize the entire compositional space. Choosing sampling points only requires finding the poles of the implicit $\chi$ function at a fixed distance from the global critical point, which we demonstrate, although we leave a full computational implementation of the compositional sampling for a large number of components to future work.

% The implicit substitution method developed in this work is a powerful technique to solve or simplify the nonlinear systems of equations encountered in the thermodynamics of solutions. The only price paid is that the derived solutions are implicit in composite composition variables, themselves a function that is a combination of the coexisting phase concentrations. Nevertheless, we expect the technique will find rich applications in thermodynamic analyses in various contexts.






% % Recently, Qian et al. proposed an iterative analytical approximation to the binodal curve for the Flory-Huggins theory \cite{qian2022analytical}, which was then used to fit experimental data. Such an approximation is very useful compared to numerical solutions, but the approach can lose accuracy at large values of polymer degree of polymerization, $N$, and polymer interactions, $\chi$, far from the critical point. Such a formulation can become a numerical exercise, or involve long analytical formulas, to reach realistic regimes and ensure accuracy. In experiments involving proteins or other polymers, the values of $N$ can become very large. Deriving a simple asymptotically accurate formula in the large $N$ limit could help fit experimental data which is often measured in this regime, far from the critical point.


% % Here, we derive an approximate solution to the Flory-Huggins model that is valid in the high $N$ limit. First, we reduce the coupled nonlinear (two-variable) Flory-Huggins model into two independent nonlinear equations, one explicit and one implicit equation. Then, we approximate the solution to the implicit equation and compare to the numerical results. 

% % The usefulness of our developments is two-fold. First, posing the mathematical problem in terms of just one nonlinear equation in one variable is intrinsically easier to solve than two coupled nonlinear equations. Second, the analytical approximation we derive is simple and reasonably accurate.






% \section{The Flory-Huggins Model: One Polymer}
% The Flory-Huggins model may be derived by a free energy density where  a polymer composed of $N$ monomers occupies a lattice. The free energy density per lattice site, $f$, may be expressed in dimensionless terms, $\tilde{f}$, as:
% \begin{equation}
% \begin{split}
%   \tilde{f}=\frac{fv}{k_BT}=&\frac{1}{N}\phi\ln(\phi)+(1-\phi)\ln(1-\phi)\\ &+\chi\phi(1-\phi)
%   \end{split}
% \end{equation}
% Here, $v$ is a lattice site volume, $k_B$ is the Boltzmann constant, $T$ is the absolute temperature,  and $\phi$ is the polymer volume fraction. $\chi$ is the so-called Flory parameter which captures the interaction between solvent and the polymer~\cite{doi2013soft}.

% From this free energy, we can define the dimensionless chemical potential of the polymer, ${\mu}=\partial \tilde{f}/\partial \phi$, up to an arbitrary constant:
% \begin{equation}
% {\mu}=\frac{1}{N}\ln(\phi)-\ln(1-\phi)-2\chi \phi.
% \end{equation}
% and the dimensionless osmotic pressure of the solution is $\tilde{\Pi}=-\tilde{f}+\phi\tilde{f}^\prime$:
% \begin{equation}
%    {\Pi}=\left(\frac{1}{N}-1\right)\phi-\ln(1-\phi)-\chi\phi^2.
% \end{equation}

% The model predicts two coexisting phases, a dense phase and a dilute phase of the polymer, above a critical $\chi$ value, $\chi>\chi_c$,
% \begin{equation}
%     \chi_c=\frac{1}{2}\left(1+\frac{1}{\sqrt{N}}\right)^2
% \end{equation}
% and above a critical polymer volume fraction $\phi >\phi_c$:
% \begin{equation}
%     \phi_c=\frac{1}{1+\sqrt{N}}
% \end{equation}
% It is found that as $N$ increases, the phase diagram becomes asymmetric relative to the center line at $\phi=1/2$. 

% Chemical equilibrium between two phases at volume fractions $\phi_A$ and $\phi_B$ is specified by two contraints---equal chemical potential of the polymer and equal osmotic pressure of the solvent:
% \begin{subequations}
%     \begin{equation}
%         \mu(\phi_A)=\mu(\phi_B)
%     \end{equation}
%     \begin{equation}
%         \Pi(\phi_A)=\Pi(\phi_B).
%     \end{equation}
% \end{subequations}

% These coupled equations can be rewritten explicitly as:
% \begin{subequations}
%     \begin{equation}\label{eq:eqChemEqA}
%         \frac{1}{N}\ln\left(\frac{\phi_A}{\phi_B}\right)-\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)-2\chi (\phi_A-\phi_B)=0 
%     \end{equation}
%     \begin{equation}\label{eq:eqChemEqB}
%         \left(\frac{1}{N}-1\right)(\phi_A-\phi_B)-\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)-\chi(\phi_A^2-\phi_B^2)=0
%     \end{equation}
% \end{subequations}

% If $\chi$ is known, then we have two equations with two unknowns, $\phi_A$ and $\phi_B$. To our knowledge, these coupled equations are impossible to deconvolve into two explicit functions describing $\phi_A$ and $\phi_B$ with known analytical techniques. However, in order to make analytical progress, we propose two simultaneous strategies. First, we search for implicit solutions, where we treat $\chi$ as an unknown, so as to gain an additional degree of freedom in the compositional space, and also since we can eliminate $\chi$ from the system of equations quite easily. Second, instead of working with the variables $\phi_A$ and $\phi_B$, we use two orthogonal composite variables that combine $\phi_A$ and $\phi_B$, which we call $y$ and $z$, that become immediately apparent after eliminating $\chi$. Thus, the problem reduces down to solving for one unknown variable, $z$, in terms of one known variable $y$. We call this solution method an implicit substitution method, since we use substitution of our implicit function $\chi$ to eliminate it. Now that the strategy has been mapped out, we implement it in detail below.



% \subsection{Analytical solution}
% First, we solve the equations \ref{eq:eqChemEqA} and \ref{eq:eqChemEqB} for $\chi$:
% \begin{subequations}
% \begin{equation}\label{eq:eqChemEqChiA}
%     \chi=\frac{\frac{1}{N}\ln\left(\frac{\phi_A}{\phi_B}\right)-\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)}{2(\phi_A-\phi_B)} 
%     \end{equation}
%     \begin{equation}\label{eq:eqChemEqChiB}
%         \chi=\frac{\left(\frac{1}{N}-1\right)(\phi_A-\phi_B)-\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)}{\phi_A^2-\phi_B^2}
%     \end{equation}
% \end{subequations}
% and equate these expressions to eliminate $\chi$, multiplying through by a factor $2(\phi_A^2-\phi_B^2)$. 
% \begin{equation}
% \begin{split}
%         &\left[\frac{1}{N}\ln\left(\frac{\phi_A}{\phi_B}\right)-\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)\right](\phi_A+\phi_B)=\\&2\left(\frac{1}{N}-1\right)(\phi_A-\phi_B)-2\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)
% \end{split}
% \end{equation}
% Organizing the terms, we can write this as:
% \begin{equation}
% \begin{split}
%         &\frac{\phi_A+\phi_B}{N}\ln\left(\frac{\phi_A}{\phi_B}\right)+(2-\phi_A-\phi_B)\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)=\\&2\left(\frac{1}{N}-1\right)(\phi_A-\phi_B),
% \end{split}
% \end{equation}
% or:
% \begin{equation}
% \begin{split}
%         &\frac{\phi_A+\phi_B}{N(\phi_A-\phi_B)}\ln\left(\frac{\phi_A}{\phi_B}\right)+\frac{2-\phi_A-\phi_B}{\phi_A-\phi_B}\ln\left(\frac{1-\phi_A}{1-\phi_B}\right)=\\&2\left(\frac{1}{N}-1\right).
% \end{split}
% \end{equation}
% If we define variables $y$ and $z$ as:
% \begin{equation}
% \begin{split}
%         &y=\frac{\phi_A-\phi_B}{\phi_A+\phi_B}\\
%         &z=\frac{\phi_A-\phi_B}{2-\phi_A-\phi_B}
% \end{split}
% \end{equation}
% the equation becomes:
% \begin{equation}
%     \frac{1}{Ny}\ln\left(\frac{1+y}{1-y}\right)-\frac{1}{z}\ln\left(\frac{1+z}{1-z}\right)=2\left(\frac{1}{N}-1\right).
% \end{equation}
% The variables $y$ and $z$ are relative measures of the partitioning of polymer and solvent, respectively, between phases, and they are already commonly used as an order parameter that defines the phase composition differences going back to Cahn and Hilliard~\cite{cahn1958free}. Since we have one degree of freedom, we will specify the variable $y$, and then solve the above equation for $z$.

% In this pursuit, we first can recognize the $\tanh^{-1}$ function, defined by the identity:
% \begin{equation}
%     \tanh^{-1}(y)=\frac{1}{2}\ln\left(\frac{1+y}{1-y}\right)
% \end{equation}
% to rewrite the above equation as:
% \begin{equation}\label{eq:eqatanh}
%     \frac{1}{Ny}\tanh^{-1}(y)-\frac{1}{z}\tanh^{-1}(z)=\frac{1}{N}-1
% \end{equation}
% % Next, if we define $x=\tanh^{-1}(z)$ and $x_1=\tanh^{-1}(y)$, then the equation becomes:
% % \begin{equation}
% %     \frac{x_1}{N\tanh(x_1)}-\frac{x}{\tanh(x)}=\left(\frac{1}{N}-1\right).
% % \end{equation}

% % Which we can write in terms of $\tanh(x)/x$:
% % \begin{equation}
% %     \frac{\tanh(x)}{x}=\left[\frac{x_1}{N\tanh(x_1)}-\left(\frac{1}{N}-1\right)\right]^{-1}
% % \end{equation}

% If we define the function $h(x)$ as:
% \begin{equation}
%     h(x)=\frac{\tanh^{-1}(x)}{x}
% \end{equation}
% equation \ref{eq:eqatanh} becomes:
% \begin{equation}
%     h(z)=1+(h(y)-1)/N
% \end{equation}

% We call this function, $h()$, the ``FH function'' since it features prominently in our solution method. Using the inverse FH function, $h^{-1}(x)$, which returns the positive branch, we can solve the equation for $z$ in terms of $y$:
% \begin{equation}\label{eq:eqZdef}
%     z=h^{-1}\left(\frac{1}{N}h(y)-\frac{1}{N}+1\right).
% \end{equation}
% Therefore, at this point, we have solved the phase diagram exactly in terms of $y$ and $z$. The function $h^{-1}(x)$ can be evaluated easily using predefined lookup tables (our strategy), though other strategies based on convergent series representations or asymptotic expressions of $h^{-1}(x)$ are possible. We leave these approaches to future practitioners if they are necessary.

% From the definition of $y$ and $z$, we can find $\phi_A+\phi_B$:
% \begin{equation}\label{eq:eqsumdef}
%     \phi_A+\phi_B=\frac{2z}{y+z}
% \end{equation}
% Finally, we can return to equation \ref{eq:eqChemEqChiB}, expressing $\chi$ in terms of $y$:
% \begin{equation}
%     \chi=\frac{\left(\frac{1}{N}-1\right)(\phi_A+\phi_B)y-\ln\left(\frac{1-z}{1+z}\right)}{(\phi_A+\phi_B)^2y}
% \end{equation}
% where we substitute in for $z$ and $\phi_A+\phi_B$ in terms of $y$ from equations \ref{eq:eqZdef} and \ref{eq:eqsumdef}.

% As mapped out in the schematic in Figure 1a, to construct the binodal curve, we specify a value of $y$ between 0 and 1. Then, we find the corresponding $\chi$ value. If we wish to cast this in terms of $\phi_A$ and $\phi_B$ we can write:
% \begin{equation}
%     \begin{split}
%         &\phi_A=\frac{z(1+y)}{z+y}\\
%         &\phi_B=\frac{z(1-y)}{z+y}
%     \end{split}
% \end{equation}
% If we enumerate multiple values of $y$ between 0 and 1, we can construct the full phase diagram. Our solution is therefore an implicit function, $\chi(y)$, which we can map to $\chi(\phi)$. Note that we do not need to explore negative values of $y$ since we arbitrarily assert that the $A$ phase is enriched in the polymer relative to the $B$ phase. 

% \begin{figure}[t]
% \centerline{\includegraphics[scale=0.25]{onecomp.png}}
% \caption{Polymer-solvent solution. Phase diagram for a single polymer-solvent solution,  comparing different degrees of polymerization ($N=10, 50, 100, 500$). The numerical solution overlaps perfectly with the exact analytical solution derived here. For large $N$, the asymptotic approximation first used by Flory~\cite{flory1942thermodynamics} matches most of the curve far from the critical point.}
% \end{figure}

% The exact solutions to the Flory-Huggins theory are plotted in Figure 2 for $N=$ 10, 50 , 100, and 500, which we confirm match numerical solutions of the coupled nonlinear equations. Interestingly, the implicit asymptotic approximation first proposed by Flory ~\cite{flory1942thermodynamics} (Appendix A) is able to capture the asymptotic behavior of the phase distribution, especially for large $N$.  It seems that this approximation has not received significant attention, since most attention has been paid to analytical approximations in the region near the critical point and extensions from the critical point. While the description in Appendix A contains more details, the crux of Flory's method was to  work with the implicit solution $\chi(\phi_A)$, taking advantage of the large asymmetry between the dense and dilute phase, $\phi_A\gg \phi_B$, to get:
% \begin{equation}
%     \chi \approx \frac{\left(\frac{1}{N}-1\right)\phi_A-\ln\left(1-\phi_A\right ) }{\phi_A^2}.
% \end{equation}
% Then, the value of $\chi$ for a given fixed value of $\phi_A$ can be used to estimate the dilute phase concentration, $\phi_B$. This approximation works especially well when there are large asymmetries in the dilute and dense phase concentrations (large $N$ and large $\chi$), and is nearly uniformly valid for large $N$.



% Now that we have solved the single-polymer case, we can turn our attention to what we can learn about multicomponent mixtures.

% \section{Multicomponent mixtures}
% Most polymer samples involve multiple polymeric species, if not by design or by impurities, then by the polydispersity of a given polymer sample---since each polymer of a specified length must be treated as a separate species. Here, we will introduce the extension of Flory-Huggins to multiple components. Then, the procedure for implementing the implicit substitution method for this system is expounded. Since the number of variables scales with the number of components, inevitably, we must introduce numerous composite variables along the way, which we define as needed. However, the strategy remains the same---working with variables $z$ and $y_i$, then using substitution of $\chi$ to arrive at one nonlinear equation with one unknown, and then specifying only the allowed number of composite variables to arrive at a valid solution.

% For a multicomponent system with $M$ polymeric species in a solvent, the free energy density is ~\cite{mao2019phase}:
% \begin{equation}
% \begin{split}
%     \tilde{f}&=\sum_i \frac{\phi_i}{N_i}\ln(\phi_i)+\left(1-\sum_i \phi_i\right)\ln\left(1-\sum_i \phi_i\right)\\
%     &-\chi \sum_i \sum_j \alpha_{ij}\phi_i\phi_j
%     \end{split}
% \end{equation}
% where the sums are over all $M$ components. The coefficients $\alpha_{ij}$ indicate the shape of the symmetric interaction matrix, while the prefactor $\chi$ measures the magnitude. We assume that the matrix $\mathbf{\alpha}$ is known.

% The chemical potential of each species, $\mu_i=\partial \tilde{f}/\partial \phi_i$, is up to an additive constant:
% \begin{equation}
%     \mu_i= \frac{1}{N_i}\ln(\phi_i)-\ln\left(1-\sum_j \phi_j\right)-\chi\sum_j 2 \alpha_{ij}\phi_j.
% \end{equation}

% The osmotic pressure of the solution is computed as $\Pi=-\tilde{f}+\sum_i \phi_i \partial \tilde{f}/\partial \phi_i$:
% \begin{equation}
%     \Pi=\sum_i\left(\frac{1}{N_i}-1\right)\phi_i-\ln\left(1-\sum_i \phi_i\right)-\chi \sum_i \sum_j \alpha_{ij}\phi_i\phi_j.
% \end{equation}

% We will assume that two phases in equilibrium have composition $\mathbf{\Phi}_A$ and $\mathbf{\Phi}_B$, where $\mathbf{\Phi}$ indicates a vector with the components consisting of the corresponding chemical volume fractions. These phases satisfy the chemical equilibrium constraints of $\mu_{iA}=\mu_{iB}$ and $\Pi_A=\Pi_B$. Here we will have $M+1$ equations and $2M+1$ unknowns ($\mathbf{\Phi}_A$ and $\mathbf{\Phi}_B$ and $\chi$). Therefore, we can set only $M$ variables independently. 

% Following the pattern from the one-component case with the implicit substitution method, we can simplify the arguments of the $\ln$ functions by defining, $y_i$:
% \begin{equation}
%     y_i=\frac{\phi_{iA}-\phi_{iB}}{\phi_{iA}+\phi_{iB}}.
% \end{equation}
% which are between -1 and 1. Arbitrarily, we choose $0\leq y_1 <1$, although all other $y_i$ can take on negative or positive values.

% The analogous variable for the solvent is $z$:
% \begin{equation}
%     z=\frac{\sum_i \left(\phi_{iA} - \phi_{iB} \right)}{2-\sum_i \left(\phi_{iA}+ \phi_{iB}\right) }.
% \end{equation}
% If we define the set of variables $\beta_i$:
% \begin{equation}
%     \beta_i=\phi_{iA}+ \phi_{iB}
% \end{equation}
% we can relate $z$ and $y_i$:
% \begin{equation}\label{eq:beta_identity}
%     \sum_i y_i \beta_i =(2-\sum_i \beta_i)z.
% \end{equation}

% To start solving the system analytically, we first solve each constraint for $\chi$. The $M$ chemical potential equations give:
% \begin{equation}
%     \chi=\frac{\frac{1}{N_i}\ln\left(\frac{1+y_i}{1-y_i}\right)-\ln\left(\frac{1-z}{1+z}\right)}{\gamma_i}
% \end{equation}
% with denominator expression, $\gamma_i$, defined as:
% \begin{equation}
%     \gamma_i=\sum_j 2 \alpha_{ij}\beta_j y_j.
% \end{equation}

% From the osmotic pressure equation, we get:
% \begin{equation}
%     \chi=\frac{\sum_i\left(\frac{1}{N_i}-1\right)\beta_i y_i-\ln\left(\frac{1-z}{1+z}\right)}{\gamma_0}
% \end{equation}
% with $\gamma_0$ defined as:
% \begin{equation}
% \begin{split}
%     \gamma_0&=\sum_i \sum_j \alpha_{ij}\left(\phi_{iA}\phi_{jA}-\phi_{iB}\phi_{jB}\right)\\
%     &=\sum_i \sum_j \alpha_{ij} y_j \beta_i \beta_j=\frac{1}{2}\sum_i \beta_i \gamma_i.
%     \end{split}
% \end{equation} 

% We can again conveniently cast the equations for $\chi$ in terms of $\tanh^{-1}$ functions:
% \begin{equation}
% \begin{split}
%     &\chi=\frac{\frac{2}{N_i}\tanh^{-1}(y_i)+2\tanh^{-1}(z)}{\gamma_i}\\
%     &\chi=\frac{2\tanh^{-1}(z)+\sum_i\left(\frac{1}{N_i}-1\right)\beta_i y_i}{\gamma_0}
% \end{split}
% \end{equation}

% For compact notation, we will define variable $x$ as:
% \begin{equation}
%     x=\tanh^{-1}(z)
% \end{equation}
% so that $z=\tanh(x)$, and variables $x_i$  as
% \begin{equation}
%     x_i=\tanh^{-1}(y_i).
% \end{equation}

% Before proceeding we can simplify the expressions for $\gamma_i$ by defining a variable $w_i$, which is a measure of the relative partitioning of component $i$ relative to the partitioning of component $1$:
% \begin{equation}
%     w_i=\frac{\beta_i y_i}{\beta_1 y_1}=\frac{\phi_{iA}-\phi_{iB}}{\phi_{1A}-\phi_{1B}}
% \end{equation}
% with $w_1=1$. The definition of $\gamma_i$ in terms of the set $w_i$ is therefore:
% \begin{equation}
% \begin{split}
%         \gamma_i&=\beta_1 y_1\sum_j 2 \alpha_{ij}w_j, \quad\quad i\neq 0 \\
%     \gamma_0&=\beta_1 y_1\sum_i \sum_j \alpha_{ij} w_j \beta_i
% \end{split}
% \end{equation}

% With the definition of $w_i$, we can solve for $\beta_i$ in terms of the set of $y_i$, $z$, and $w_i$ by applying equation \ref{eq:beta_identity}:
% \begin{equation}\label{eq:beta_defined}
%     \beta_i=\frac{2 z w_i}{y_i\sum_j\left[w_j\left(1+\frac{z}{y_j}\right)\right]}
% \end{equation}

% The next step, using our favorite implicit substitution method, is to equate the equations for $\chi$. For this purpose, we will first equate the $\chi$ from the first component to all other components, for $M-1$ equations. Then we will equate a convenient linear combination of $\chi$ from all components to the $\chi$ specified by the osmotic pressure, in order to cancel the denominator $\gamma_0$. 

% The combined chemical potential equations give:
% \begin{equation}
%         \frac{\frac{2}{N_i}x_i+2x}{\gamma_i}=\frac{\frac{2}{N_1}x_1+2x}{\gamma_1}.
% \end{equation}
% which rearranged is:
% \begin{equation}
%     x_i=x\left(\frac{\gamma_i}{\gamma_1}-1\right)N_i+\frac{\gamma_i}{\gamma_1} \frac{x_1 N_i}{N_1}.
% \end{equation}

% We can next apply the osmotic pressure constraint on $\chi$, which we write as:
% \begin{equation}
%     \frac{2x+ \sum_j\left(\frac{1}{N_j}-1\right)\beta_j y_j}{\gamma_0}=\frac{\frac{2}{N_i}x_i+2x}{\gamma_i}.
% \end{equation}
% We can multiply this equation by $\beta_i\gamma_i$, then sum over all components:
% \begin{equation}
%     \frac{\sum_i \beta_i\gamma_i}{\gamma_0} \left(2x+ \sum_j\left(\frac{1}{N_j}-1\right)\beta_j y_j\right)=\sum_i\beta_i\left(\frac{2x_i}{N_i}+2x\right).
% \end{equation}
% Applying the definition of $\gamma_0$ so as to eliminate it:
% \begin{equation}
%      \left(2x+ \sum_j\left(\frac{1}{N_j}-1\right)\beta_j y_j\right)=\sum_i\beta_i\left(\frac{x_i}{N_i}+x\right).
% \end{equation}
% Then, collecting terms in $x$, we get:
% \begin{equation}
%     \left(2-\sum_i\beta_i\right)x-\sum_i\beta_i y_i=\sum_i \frac{\beta_i x_i}{N_i}-\frac{\beta_i y_i}{N_i},
% \end{equation}
% which can be written compactly as:
% \begin{equation}
%      \left(2-\sum_i\beta_i\right)(x-z)=\sum_i \frac{\beta_i(x_i-y_i)}{N_i}
% \end{equation}
% or as:
% \begin{equation}
%     \frac{x}{z}=1+\frac{\sum_i \beta_i(x_i-y_i)/N_i}{\sum_i \beta_i y_i}.
% \end{equation}
% Further substituting in for $\beta_i$ from equation \ref{eq:beta_defined} gives:
% \begin{equation}
%     \frac{x}{z}=1+\frac{\sum_i w_i(x_i/y_i-1)/N_i}{\sum_i w_i}
% \end{equation}
% We can again write this expression in terms of the FH function, $h()$:
% \begin{equation}\label{eq:masterequation}
%     h(z)=1+\frac{\sum_i w_i(h(y_i)-1)/N_i}{\sum_i w_i}
% \end{equation}
% Defining $\eta_i=\gamma_i/\gamma_1$, the chemical potential constraints on $\chi$ give:
% \begin{equation}
%     x_i=N_i(\eta_i-1)x+\eta_i N_ix_1 /N_1
% \end{equation}
% or in terms of $y_i$:
% \begin{equation} \label{eq:eqyidefined}
%     y_i=\tanh(N_i(\eta_i-1)\tanh^{-1}(z)+\eta_i N_i\tanh^{-1}(y_1) /N_1)
% \end{equation}

% At this stage, by substituting in equation \ref{eq:eqyidefined} into equation \ref{eq:masterequation}, and specifying the $M$ composite variables $y_1$ and $w_i$ for $i>1$, we have successfully transformed our system of $M+1$ equations into one master equation, equation \ref{eq:masterequation}, in one unknown, $z$, the solvent partitioning between phases. However, this equation does not have a clear inversion formula, since $z$ is contained differently as an argument of multiple nonlinear functions, not just one nonlinear function as in the one polymer case. Therefore, in the most general case, the master equation must be solved numerically. Note however, that there are clear strategies to approximate the master equation solution near and far from the critical point, as outlined in Appendices A and B.

% \begin{figure*}[t!]
% \centerline{\includegraphics[scale=0.2]{polydisperse.png}}
% \caption{Polydisperse polymer-solvent solution. Comparison of the phase diagram for two polydisperse samples composed of one polymer type. (a) Coexistence curves plotting $\chi$ versus total volume fraction of polymer $\phi=\sum_i \phi_i$. Each curve fixes the volume fraction of the condensed phase, $\nu$. The binodal curves are calculated with a polymer with a uniform molecular weight distribution between $N=10-100$, and separately for a polymer with an exponential molecular weight distribution between $N=10-100$, $\bar{\phi}_i/\bar{\phi}_1=\exp((N_i-10)/45)$. (b-c) The molecular weight distributions of the overall solution (thick lines), and the molecular weight distributions in the dense and dilute phase at $\chi=0.8$. Note that for $\nu=0$ and $\nu=1$, the dilute and dense phase, respectively, perfectly overlap with the overall molecular weight distribution.}
% \end{figure*}

% To solve this system of equations with the maximum of $M$ specified variables, we choose the set of $w_i y_1$ for $i>1$ and $y_1$, so that the specified variables have the same denominator of $\phi_{1A}+\phi_{1B}$, and so that they all go to zero at the global critical point. From $w_i$, one can determine the set $\eta_i$. Then, the master equation can be solved for $z$ numerically. With $z$ in hand, then all values of $y_i$ and $\beta_i$ can be calculated explicitly, then finally $\chi$ can be calculated using one of the original equilibrium constraints.

% Even though a numerical solution of the master equation is still needed in general, a vast simplification has been achieved by all the algebraic manipulations entailed by the implicit substitution method--- turning the system of $M+1$ nonlinear equations into one nonlinear master equation with one unknown. Again, we must work with the composite variables $y_1$ and $w_i$, but as sketched out in the schematic in Figure 1b and c, the solution can be directly transformed back to $\mathbf{\Phi}$ space with the relation:
% \begin{subequations}
%     \begin{equation}
%         \phi_{iA}= \frac{1}{2}\beta_i(1+y_i)
%     \end{equation}
%     \begin{equation}
%         \phi_{iB}=\frac{1}{2}\beta_i(1-y_i)
%     \end{equation}
% \end{subequations}
% Additionally, we must also check that the solutions returned are actually physical, since admissible solutions to the master equation can return negative values of the densities.


% In what follows, we discuss applications of the multicomponent solution method to three special cases. The first case is that of a single polymer with an arbitrary number of different lengths (known as polydispersity). There, we find an exact analytical solution, and the master equation solution can be completely cast in terms of two independent variables without any numerical solution necessary. In the second case, we apply the solution method to a two polymer, one solvent system, to demonstrate how the method can be used to find the $\chi$ function over the full compositional space. Finally, in the third case, we suggest strategies to tackle the problem of large multicomponent systems of polymers using the implicit solution without discretizing the entire composition space.





% % Next, define the variable $\theta_i=w_i/\sum_i w_i$, to give $\eta_i$:
% % \begin{equation}
% %     \eta_i= \theta_i(x_i/y_i-1)/N_i
% % \end{equation}
% % that can be substituted in to give:
% % \begin{equation}
% %     \frac{x}{z}=1+\sum_i \eta_i
% % \end{equation}
% % We can write the constraint for chemical potential now in terms of $\theta_j$:
% % \begin{equation}
% %     \frac{\gamma_i}{\gamma_1}=\frac{x_i/N_i+x}{x_1/N_1+x}=\frac{\sum_j\alpha_{ij}\theta_j}{\sum_j\alpha_{1j}\theta_j}
% % \end{equation}

% % \begin{equation}
% %     \frac{\sum_i \theta_i x_i/(y_i N_i)+ \sum_i \theta_i x}{x_i/N_i+x}=\frac{\sum_i\sum_j\theta_i\alpha_{ij}\theta_j}{\sum_j\alpha_{ij}\theta_j}
% % \end{equation}



% % \begin{equation}
% %   \frac{x_i \gamma_1}{N_i}-\frac{x_1 \gamma_i}{N_1}+x(\gamma_1-\gamma_i)=0
% % \end{equation}
% % Substitution of $\gamma$ gives:
% % \begin{equation}
% %     \sum_j \left[\frac{x_i}{N_i}\alpha_{1j} -\frac{x_1}{N_1}\alpha_{ij}+ x\left(\alpha_{1j}-\alpha_{ij}\right)\right]w_j=0
% % \end{equation}
% % In these equations, $w_i$ appears linearly, and we can solve this linear system of equations to arrive at $w_i(x)$ directly, maintaining the $x$ dependence. The determinant of the matrix of $N-1$ equations is a polynomial in $x$ of order $x^{N-1}$. Therefore, without fortuitous cancellations, we expect that the $w_i$ functions will be rational functions of order $x^{N-1}$.

% % At this stage, the final unknown is $x$. To specify this variable, we must solve for the $\chi$ value from the osmotic pressure.
% % \begin{equation}
% %     \frac{2x+\beta_1 y_1 \sum_i\left(\frac{1}{N_i}-1\right)w_i}{\gamma_0}=\frac{\frac{2}{N_1}x_1+2x}{\gamma_1}
% % \end{equation}
% % This can be rewritten as:
% % \begin{equation}
% %     \frac{1}{2}\sum_i\left(\frac{1}{N_i}-1\right)w_i=\frac{x}{\beta_1 y_1}\left(\frac{\gamma_0}{\gamma_1}-1\right)+\frac{x_1}{\beta_1 y_1 N_1}\frac{\gamma_0}{\gamma_1}
% % \end{equation}
% % From the definition of $\gamma$, we have:
% % \begin{equation}
% % \begin{split}
% %     \frac{\gamma_0}{\gamma_1\beta_1 y_1}&=\frac{\sum_i \sum_j \alpha_{ij} w_j \beta_i}{\beta_1 y_1\sum_j 2 \alpha_{1j}w_j}\\
% %     &=\frac{\sum_i \sum_j \alpha_{ij} w_j \frac{z w_i}{y_i}}{\beta_1y_1\left(\sum_j  \alpha_{1j}w_j\right)\left(\sum_j\left[w_j\left(1+\frac{z}{y_j}\right)\right]\right)}\\
% %     &=\frac{\sum_i \sum_j \alpha_{ij} w_j \frac{z w_i}{y_i}}{2z\left(\sum_j  \alpha_{1j}w_j\right)}\\
% %     &=\frac{\sum_i \sum_j \alpha_{ij} w_j w_i/\tanh(x_i)}{2\left(\sum_j  \alpha_{1j}w_j\right)}
% %     \end{split}
% % \end{equation}
% % and we also know:
% % \begin{equation}
% % \begin{split}
% %     \frac{1}{\beta_1 y_1}&=\frac{\left(\sum_jw_j\right)+z\left(\sum_j w_j/y_j\right)}{2z}\\
% %     &=\frac{\sum_jw_j}{2\tanh(x)}+\sum_j \frac{w_j}{2\tanh(x_j)}
% % \end{split}
% % \end{equation}
% % Now we rewrite the master equation as:
% % \begin{equation}
% % \begin{split}
% %     &\frac{1}{2}\sum_i\left(\frac{1}{N_i}-1\right)w_i-\frac{1}{\beta_1 y_1}\frac{\gamma_0}{\gamma_1}\left(x+\frac{x_1}{N_1}\right) \\ 
% %     &+x\sum_j \frac{w_j}{2\tanh(x_j)} =-\frac{x\sum_jw_j}{2\tanh(x)}
% % \end{split}
% % \end{equation}

% % Finally, we can solve the equation for $\tanh(x)/x$:




% % \begin{widetext}
% % \begin{equation}
% % \begin{split}
% %         \frac{\tanh(x)}{x}&=\frac{\sum_j w_j}{\frac{\sum_i \sum_j \alpha_{ij} w_j w_i/\tanh(x_i)}{\left(\sum_j  \alpha_{1j}w_j\right)}\left(x+\frac{x_1}{N_1}\right)-\sum_j\left[\left(\frac{1}{N_j}-1\right)w_j+\frac{x w_j}{\tanh(x_j)}\right]}\\
% %         \frac{\tanh(x)}{x}&=\frac{\left(\sum_j w_j\right)\left(\sum_j  \alpha_{1j}w_j\right)}{\sum_i \sum_j \frac{\alpha_{ij} w_j w_i}{\tanh(x_i)}\left(x+\frac{x_1}{N_1}\right)-\sum_j\left[\left(\frac{1}{N_j}-1\right)w_j+\frac{x w_j}{\tanh(x_j)}\right]\left(\sum_j  \alpha_{1j}w_j\right)}
% % \end{split}
% % \end{equation}
% % \end{widetext}

% % From the above equation, we see that $\tanh(x)/x=R(x)$, where $R(x)$ is a rational function with all variables but $x$ known. Generally speaking, this equation must be solved numerically, unless there is some fortuitous simplification. That being said, we have simplified the equations considerably by getting to this point. Furthermore, additional phase coexistences (more than two phases) correspond to more than one solution to the above master equation.





% \subsection{Polydisperse polymer of one type}
% If a solution consists of only a solvent and only one polymer of one type, but that polymer is polydisperse which gives distinct values of $N_i$, then we can often assume the interactions are equal for each length of polymer, i.e. $\alpha_{ij}=1$, which means that $\eta_i=1$ for all $i$. In this case, the value of $y_i$ becomes independent of $z$:
% \begin{equation}
%     y_i=\tanh\left(\frac{N_i}{N_1}\tanh^{-1}(y_1)\right).
% \end{equation}
% If this is the case, then we can again solve the equation for $z$ explicitly with the inverse FH function $h^{-1}$, exactly as we did for the one component case:
% \begin{equation}
%     z=h^{-1}\left(1+\frac{\sum_i w_i(h(y_i)-1)/N_i}{\sum_i w_i}\right)
% \end{equation}

% For arbitrary molecular weight distributions, the values of $w_i$ and $y_1$ can be chosen independently to construct the full phase diagram. However, in many cases, the molecular weight distribution of the polymer being added to the solvent is known. If the average volume fraction of a particular molecular weight in both phases, $\bar{\phi}_i$, can be written in terms of $\nu$, the volume fraction of the phase $A$ relative to the total volume:
% \begin{equation}
%     \bar{\phi}_i=\nu \phi_{iA}+(1-\nu)\phi_{iB}=(\phi_{iA}-\phi_{iB})\left(\nu+\frac{1}{2 y_i}-\frac{1}{2}\right)
% \end{equation}
% then the ratio between the average polymer density $\bar{\phi}_i/\bar{\phi}_1$ is:
% \begin{equation}
%     \frac{\bar{\phi}_i}{\bar{\phi}_1}=\frac{\left(\nu+\frac{1}{2 y_i}-\frac{1}{2}\right)}{\left(\nu+\frac{1}{2 y_1}-\frac{1}{2}\right)}w_i.
% \end{equation}
% Or solving for $w_i$, we get:
% \begin{equation}
%     w_i=\frac{\bar{\phi}_i}{\bar{\phi}_1}\frac{\left(\nu+\frac{1}{2 y_1}-\frac{1}{2}\right)}{\left(\nu+\frac{1}{2 y_i}-\frac{1}{2}\right)}.
% \end{equation}

% If $y_1$ and $\nu$ are specified, then the set $w_i$ is also fixed if the overall molecular weight distribution is known. Therefore, we can reduce the dimensionality of the phase diagram by only varying $y_1$ and $\nu$ in the ranges $0<y_1<1$ and $0<\nu<1$, as schematically sketched out in Figure 1b.

% In Figure 3, we present the phase diagram for two polymer samples of different overall molecular weight distributions, one that is uniformly distributed between $N=10-100$ and one that is exponentially distributed between $N=10-100$. These curves are analytically calculated in Figure 3a, much better than working with the 92 nonlinear chemical equilibrium equations we started with. The curves are plotted as $\chi$ versus the overall polymer volume fraction, $\phi=\sum_i \phi_i$, at fixed condensed phase volume fraction, $\nu$. In Figure 3b-c, the molecular weight distributions of the samples and the molecular weight distribution of the coexisting phases are plotted in the form of a probability density function. When the dense polymer phase volume fraction is small ($\nu\approx 0$), the binodal is pushed towards lower overall polymer density, because the first appearing condensed phases preferentially include polymers of higher molecular weight---so they dominate the coexistence curve. 

% As the volume fraction of the condensed phase, $\nu$, increases, the left branch of the coexistence curve shifts to the right, since the condensed phase is forced to more closely match the overall molecular weight distribution as the condensed phase volume fraction increases. Although $\nu\approx 1$ may be practically infeasible to reach, there, the minority dilute phase must enrich polymers of low molecular weight since they are heavily crowded in the dense phase. Note that at $\nu=0$ and $\nu=1$, the molecular weight distribution of the dilute and dense phase, respectively, perfectly match the molecular weight of the overall polymer sample. Finally, comparing the two overall molecular weight distributions, the sample more enriched in the longer polymers has a left branch of the coexistence curve shifted to the left. In all cases, the critical point appears to be dominated by the longest polymer constituents, although it varies with the specific details of the molecular weight distribution and value of $\nu$.


% \begin{figure*}[t!]
% \centerline{\includegraphics[scale=0.6]{Fig4Draft.png}}
% \caption{A two-polymer-one-solvent system. Parts (a-c) correspond to the phase diagram for a diagonally dominant interaction matrix, while parts (d-f) show the same results for an off-diagonally dominant interaction matrix. (a) The full phase diagram mapping the $\chi$ surface for all compositional space for fixed $\alpha_{ij}$ on the $y_1$, $\tanh(y_1 w_2)$ plane. All regions connect at the critical point at $y_1=0$ and $ y_1 w_2=0$, but are segmented by the singular curves on the $\chi$ surface that are evident by thick black regions on the $\chi$ surface. The three poles are computed on a small circle near the critical point, and marked with white markers. These poles can be used to demarcate the distinct differentiable regions of the $\chi$ surface. Note that the colormap is saturated at the bounds of the color bar, and while the contours lines are linear between $\chi=0$ and $\chi=4$, they are non-evenly spread out at larger or smaller values of $\chi$. (b) The regions of the $\chi$ surface which are physical, with positive predicted polymer densities. (c) The binodal curve for fixed values of $\chi$ transformed to $\mathbf{\Phi}$ space, either mapped out by the gradient descent algorithm in Section  IIIC or by extracting contours from the physical regions of the $\chi$ surface in part 4b. Parts (d-f) show the same information as (a-c), but for a different interaction matrix. }
% \end{figure*}



% % If this is the case, the $N-1$ equation for $w_i$ when $i>1$ becomes:
% % \begin{equation}
% %     \left[\frac{x_i}{N_i} -\frac{x_1}{N_1}\right] \sum_j w_j=0
% % \end{equation}
% % which are actually linearly dependent in $w$. This degeneracy arises because the excess chemical potential for each component is identical, meaning that each equation does not add new information. 

% % By the prefactor in the above equation, we see that the $x_i$ of each component is not independent, irrespective of the values of $w_i$. Therefore, it is more natural for this problem if we change out the specified variables. Instead of specifying $x_i$ for $i>1$, we can instead specify fixed values of $w_i$ for $i>1$. Then, we can simply solve for each unknown $x_i$ using the above equation:
% % \begin{equation}
% %     x_i=\frac{x_1N_i}{N_1}.
% % \end{equation}

% % Finally from the equation for the osmotic pressure, we get:
% % \begin{equation}
% % \begin{split}
% %         &\frac{\tanh(x)}{x}=\frac{\left(\sum_j w_j\right)}{\frac{x_1}{N_1}\sum_j\frac{ w_j}{\tanh(x_j)}-\sum_j\left[\left(\frac{1}{N_j}-1\right)w_j\right]}
% % \end{split}
% % \end{equation}
% % where all variables are known on the right hand side. This is an equivalent problem to the one for the one-polymer in solvent problem, where only the inverse of $\tanh(x)/x$ must be computed for the final solution. 

% % If we multiply through by the denominator, then we have a linear set of N-2 equation for $w_k$ with $k>2$ so that we can solve for these variables in terms of $z=\tanh(x)$, and an additional equation that $w_1=1$. Finally, we can solve for $z$ using the equation for $k=1$, though this will again be in the form $\tanh(x)=R(x)$ where $R(x)$ is a rational function, where $x$ only appears as $\tanh(x)$.

% % This problem highlights the issues when the $\alpha$ matrix is not in full rank. For any linearly dependent rows, we must resort to using the osmotic pressure $\chi$ equation, which is more complex.



% \subsection{A two polymer, one solvent mixture}
% While we were able to find an exact analytical solution for an arbitrarily polydisperse polymer, the two polymer-one solvent mixture has a master equation that can only be solved numerically. Here the master equation becomes:
% \begin{equation}
%     h(z)=1+\frac{(h(y_1)-1)/N_1+w_2(h(y_2)-1)/N_2}{1+w_2}
% \end{equation}
% with $y_2$ fixed as:
% \begin{equation}
%     y_2=\tanh(N_2(\eta_2-1)\tanh^{-1}(z)+\eta_2 N_2\tanh^{-1}(y_1) /N_1)
% \end{equation}
% and $\eta_2$ defined as:
% \begin{equation}
%     \eta_2=\frac{\alpha_{12}+\alpha_{22}w_2}{\alpha_{11}+\alpha_{12}w_2}
% \end{equation}

% To construct a phase diagram, we specify $y_1$ and $y_1 w_2$, then solve for $\eta_2$, then for $z$ solving the master equation numerically. From there, we can specify $y_2$, $\chi$, and then solve explicitly for the polymer densities in each phase. To discretize the phase diagram, we vary $0<y_1<1$ and $-1<\tanh(y_1 w_2)<1$. Note that it is more regularly behaved to plot the phase diagram in terms of $y_1$ and the product $y_1 w_2$, since they share the same denominator in terms of their $\mathbf{\Phi}$ dependence.

% In Figure 4, we present the solution for a two polymer-one solvent system for two different shapes of the interaction matrix: (a-c) a diagonally dominant interaction matrix and (d-f) an off diagonal dominant matrix. So as to not push the coexisting densities to extreme values near 0 or 1, we choose $N_1=4$ and $N_2=3$ as a starting point. The $\chi$ surface is calculated over the full compositional landscape. Interestingly, all differentiable regions emanate from the central critical point at $y_1=0$, $w_2y_1=0$, but are separated by singular discontinuous curves in the phase diagram. Not all of these regions or parts of these regions return physical, positive densities, as shown in Figure 4b and 4e. Nevertheless, by transforming specified contours with admissible solutions to $\mathbf{\Phi}$ space, we can map out the phase coexistence curves in terms of $\phi_1$ and $\phi_2$, as demonstrated in Figure 4c and 4f.

% Clearly for $M=2$, if the value of the desired $\chi$ contour is known, mapping out the full $\chi$ landscape may be more computationally expensive than solving the equations in $\phi$ space for the fixed, desired value of $\chi$. So the fully discretized $\chi$ surface implemented here are of limited use for generating single binodal curves at fixed $\chi$.

% A natural question at this point to ask is: how can one efficiently sample the implicit $\chi$ surface to find a desired contour or sets of contours corresponding to multiple coexisting phases?  Further, how can one choose sampling points so as to dodge the singular curves in the phase diagram? Finally, can the sampling be efficiently scaled for large values of $M$? To explore these questions, in the next section, we formulate such a sampling strategy.



% \subsection{Finding contours in a high dimensional phase diagram}
% In the case of a high dimensional multicomponent solution, we have found an implicit solution for $\chi$, requiring only one nonlinear solve in one variable, $z$, to construct the surface:
% \begin{equation}
%     \chi=\chi(y_1, \tanh(y_1 w_i))=\chi(\mathbf{v}),
% \end{equation}
% where only the $M$ independent variables are listed as arguments in the vector $\mathbf{v}$.

% Without enumerating all possible inputs for the implicit function $\chi$, we may not know beforehand where a given contour lies on the $\chi$ surface corresponding to coexisting phases. If we wish to only find the contours of this surface at fixed $\chi=\chi_0$ with minimal number of $\chi$ evaluations in a high dimensional phase diagram ($M\gg 1$), then we can employ a gradient descent algorithm on the $\chi$ surface to arrive at the desired contour. Defining the inputs of the $\chi$ function as a vector $\mathbf{v}$, with step index $k$, the algorithm proceeds as:
% \begin{equation}
%     \mathbf{v}_{k+1}=\mathbf{v}_k-\lambda_k \nabla_v F(\mathbf{v}).
% \end{equation}
% The function $F$ is:
% \begin{equation}
%     F(\mathbf{v})=\left(\chi(\mathbf{v})-\chi_0\right)^2,
% \end{equation}
% and its gradient can be computed by finite difference. The step size $\lambda_k$ can be specified by a given algorithm, such as the Barzilai-Borwein method~\cite{barzilai1988two}. 

% % Other algorithms such as Newton's method could be employed with the extra expense of calculating the Hessian matrix at each iteration.

% Once the desired contour is reached, one can then trace out a contour by stepping along a direction, $\mathbf{u}$, perpendicular to the gradient $\mathbf{g}=\nabla_v \chi$:
% \begin{equation}
% \mathbf{v}_{k+1}=\mathbf{v}_k-\lambda_k \mathbf{u}
% \end{equation}
% with 
% \begin{equation}
% \begin{split}
%         &u_i=g_i, \quad \quad i>1 \\
%         &u_i=-\frac{1}{g_1}\sum_{i>1} g_i^2 \quad \quad i=1
% \end{split}
% \end{equation}

% Here the step size $\lambda_k$ can be scaled by the magnitude of the gradient vector or the location of the current iteration, $\mathbf{v}_k$. If ever the step size is too large and the algorithm steps off of the fixed $\chi$ contour, the gradient descent can be used to return to the contour.  

% Such an algorithm works to converge to one contour in the $\mathbf{v}$ space, corresponding to phase coexistence points in the $\mathbf{\Phi}$ space. If the algorithm is initiated in a region that is separated from the desired contour by a singular, non-differentiable curve in the $\mathbf{v}$ space, then more than one starting point would be needed to locate all matching contours in the phase diagram. If this is the case, then it is natural to ask: what are efficient ways to choose candidate starting points?

% Notably, all regions connect at the global critical point at $\mathbf{v}=0$, but the regions are separated by singularities which extend radially from the critical point, slicing the phase diagram like a pie, as seen clearly in Figures 4a and 4d. Therefore, the analytical approximations of the equations by expanding near the critical point and finding poles can give a small number of candidate starting points in each region located at the center of each pie piece.

% To sketch out the strategy to initiate a gradient descent algorithm, we next turn to how to segment the phase diagram efficiently to generate candidate starting points near the critical point.

% \subsubsection{Segmenting a hypersphere near the critical point}
% Near the critical point, the partitioning of each species becomes negligible, i.e., $\mid y_i\mid, \mid z\mid \ll 1 $, and the master equation is:
% \begin{equation}\label{eq:eqCrit}
%     z^2=\frac{\sum_i w_i y_i^2/N_i}{\sum_i w_i}
% \end{equation}
% with the chemical potential constraint setting:
% \begin{equation}
%     y_i=N_i(\eta_i-1)z+\eta_i \frac{N_i}{N_1} y_1
% \end{equation}
% Combined, these equations give a quadratic equation for $z$ which can be solved exactly, as documented in Appendix B. Nevertheless, extra degrees of freedom are still specified by the set $y_1$, $w_i$. 

% To eliminate these degrees of freedom, we propose the following strategy. We look for candidate starting points on a small hypersphere $\mid \mathbf{v}\mid=v_0$ near the critical point, with $v_0\ll 1/\max(N_i)$. First, we find the poles of the $\chi$ function on this hypersphere. Then, we choose a small number of points in regions demarcated by the poles of the $\chi$ function. By choosing specified points between the poles, we guarantee that we are testing each candidate region for the specified $\chi$ value. 

% For finite but small $z$ and $y_i$, the poles of the $\chi$ function are defined by the equation:
% \begin{equation}
%     \gamma_i\propto\sum_j \alpha_{ij} w_j=0 
% \end{equation}
% which corresponds to finding the null space of the $\mathbf{\alpha}$ matrix, and then rescaling so that $w_1=1$. If $\mathbf{\alpha}$ is full rank, then the null space is empty. However, one other denominator in the full expressions can go to zero, causing singularities in the phase diagram, namely:
% \begin{equation}
%     \sum_j\left[w_j\left(1+\frac{z}{y_j}\right)\right]=0
% \end{equation}
% Near the critical point, these poles must be solved for numerically for the values of $w_i$ and $y_1$ that lead to singularities, making use of the exact solution for $z$ near the critical point. 

% Note that the poles can actually be interpreted as curves on a given hypersphere. For $M=2$, they correspond to points on a circle. For $M=3$, they correspond to arcs on a sphere, and so on. In order to segment the space in higher dimensions, one would need to find the intersection of these singular curves on the hypersphere near the critical point, to find the boundaries of the nonsingular ``continents'' on the hypersphere.

% Once we have found the poles near the critical point at fixed $v_0$, we can segment the hypersphere radially between these poles, making sure to test at least one point in the gradient descent algorithm in each ``continent" of the segmented hypersphere. This would ensure that our algorithm can find a desired contour, if it exists, and could find multiple contours of the same function (multiple coexisting phases) that are separated by non-differentiable curves.
% \subsubsection{Applying the gradient descent algorithm}

% Here, we explicitly apply the gradient descent algorithm only for $M=2$, to find the contours in Fig. 4c and 4f, validating the results by comparison to the full $\chi$ surface. The poles of the function do segment the phase diagram for $M=2$, as demonstrated by the white points marked in Figure 4a and 4d on a circle a fixed distance from the critical point. Choosing a handful of starting values between the singular points on the circle, we can trace out the fixed values of $\chi$, and then transform to $\mathbf{\Phi}$ space, to identify curves matching Fig. 4c and 4f.

% While we demonstrate the gradient descent algorithm for $M=2$, we leave the exploration of $M>2$ to future work. Note that this gradient descent algorithm is very advantageous for cases where $M>4$, where it may be difficult to discretize the $\mathbf{v}$ space over the whole compositional range a priori. In fact, while the number of function evaluations at each point scales with $M$ (to evaluate the components of the gradient vectors), and the number of candidate points may also increase with $M$, the gradient descent algorithm is otherwise insensitive to $M$, which is much more favorable than discretizing all combinatoric possibilities in composition space.



% % If we fix the value of $\chi=\chi_0$, by the osmotic pressure constraint:
% % \begin{equation}
% %     \chi_0=\frac{2z+\beta_1 y_1\sum_j \left(\frac{1}{N_j}-1\right)w_j}{\beta_1 y_1\sum_i\sum_j \beta_i\alpha_{ij}w_j}
% % \end{equation}
% % and substitute $\beta_i$:
% % \begin{equation}
% %     \frac{4z^2\chi_0\sum_i\sum_j w_i\alpha_{ij}w_j/y_i}{\sum_j\left[w_j\left(1+\frac{z}{y_j}\right)\right]^2}=2z+2z\frac{\sum_j \left(\frac{1}{N_j}-1\right)w_j}{\sum_j\left[w_j\left(1+\frac{z}{y_j}\right)\right]}
% % \end{equation}
% % and simplify:
% % \begin{equation}
% %     2\chi_0\sum_i\sum_j w_i\alpha_{ij}w_j (z/y_i)=
% % \end{equation}



% % If we do the same substitution for each of the chemical potential constraints:
% % \begin{equation}
% %     \chi_0=\frac{y_i/N_i+z}{\beta_1 y_1\sum_j \alpha_{ij}w_j}=\frac{\left(y_i/N_i+z\right)\sum_j w_j\left(1+\frac{z}{y_j}\right)}{2 z\sum_j \alpha_{ij}w_j}
% % \end{equation}
% % and rearrange:
% % \begin{equation}
% %     2\chi_0 \sum_j \alpha_{ij}w_j=\left(\frac{1}{N_i}\frac{y_i}{z}+1\right)\sum_j w_j\left(1+\frac{z}{y_j}\right)
% % \end{equation}






% \section{Conclusions}
% Using the implicit substitution method, for the first time, we are able to analytically define the coexistence curves for a polymer-solvent system and a polydisperse polymer-solvent system. Such a solution will open up more opportunities to apply thermodynamic modeling in diverse applications in polymer science.

% For generalized mixtures of many components, we have simplified a large system of nonlinear equations into one nonlinear equation. We have mapped out these solutions for two polymeric components over the full compositional space, and demonstrated the demarcation between differentiable regions of the $\chi$ surface that defines the binodal curve. Further, we have suggested strategies to find full binodal curves at fixed $\chi$ without discretizing the full compositional space, which we believe will be very useful for $M>4$, but we leave a full exploration of these methods to future studies. 

% Ample opportunities exist to develop the methods presented here further. Beyond improving the computational performance of the method, one could seek analytical perturbative series solutions to the general master equation. Further, one could implement the method to large multicomponent mixtures, and explore the shape of contours of the $\chi$ surface for different interaction matrices. Moreover, the approach can be directly extended to more detailed equations of state beyond Flory-Huggins, although neat analytical solutions of a final master equation are not guaranteed for all equations of state.  In Appendix C, we highlight possible extensions of the implicit substitution method to other equations of state.

% The implicit substitution method, while possibly un-intuitive at first sight, has given us a new lens to explore the phase behavior of polymeric phase separation. We demonstrated its power in simplifying systems of coupled nonlinear thermodynamic equations that are often impossible to solve explicitly. 





% \appendix
% \section{Approximations far from the critical point}
% \subsection{Extending Flory's approximation}
% Interestingly, in his 1942 article, Flory solved his theory in a rather ingenious way~\cite{flory1942thermodynamics} using an asymptotic arguments of the osmotic pressure difference between solutions. Recognizing that the osmotic pressure of the dilute phase would go to zero relative to the condensed phase, Flory solved the osmotic pressure equation for $\chi$ keeping only terms containing the condensed phase volume fraction. Specifically, he recognized that in the limit $N\gg 1$, and away from the critical point, it is natural to expect that $\phi_B \ll 1$, i.e., the solution is very dilute in polymer, and $\phi_A\approx 1$, i.e., the second phase is rich in polymer. In this limit, it follows that equation (\ref{eq:eqChemEqB}) simplifies to: % (note that $\phi_B\ll \phi_A\approx 1$ and $\ln\left(1-\phi_B\right )\approx -\phi_B$) 
% \begin{equation}\label{eq:eqChemEq2}
%     \left(\frac{1}{N}-1\right)\phi_A-\ln\left(1-\phi_A\right ) -\chi\phi_A^2=0,
% \end{equation}
% In other words, there is an implicit relation giving $\phi_A(\chi, N)$ in the form
% \begin{equation}\label{eq:eqChemEq3}
%     \chi = \frac{\left(\frac{1}{N}-1\right)\phi_A-\ln\left(1-\phi_A\right ) }{\phi_A^2}.
% \end{equation}
% Flory used this relationship in order to approximate the $\chi$ that corresponds to a given dense phase concentration ($\phi_A$), then iteratively solved for the dilute phase concentration  ($\phi_B$) using the chemical potential constraint.

% Interestingly, the starting approximation in \ref{eq:eqChemEq3} can be applied to the chemical potential equation directly to arrive at an implicit approximation for the coexistence curve far from the critical point. The same approximation that $\phi_A\gg \phi_B$ is now applied to the chemical potential constraint in equation (\ref{eq:eqChemEqChiA}) to obtain an expression for the dilute volume fraction $\phi_B$,
% \begin{equation}\label{eq:eqChemEq4}
% \frac{1}{N} \ln \phi_B  = \frac{1}{N}\ln\phi_A - \ln\left (1-\phi_A\right )-2\chi \phi_A
% \end{equation}or 
% \begin{equation}\label{eq:eqChemEq5}
% \phi_B = \frac{\phi_A}{\left (1-\phi_A\right )^N}e^{-2N\chi \phi_A},
% \end{equation}where  $\chi$ for a specified $\phi_A$ is given in (\ref{eq:eqChemEq3}).
% This last result illustrates that typically $\phi_B$ is exponentially small.

% As seen in Figure 2, this asymptotic formula works incredibly well to describe the coexisting phases, especially for large $N$, with the exception of a small region near the critical point.



% \subsection{Approximation for multicomponent mixtures}
% On the other hand, for multicomponent mixtures, it may be difficult to seek approximations, since multiple assumptions of limiting values of densities may need to be made simultaneously, especially if multiple species co-accumulate in the condensed phase. While the limiting solution near the critical point is analytical   (by applying the quadratic formula in equation \ref{eq:eqCrit}), one general approximation does not work in all regions far from the critical point. 

% However, we can explore the limiting behavior when the major component, which we arbitrarily specify as component 1, has a large excess in the condensed phase compared to the dilute phase relative to other components. We also choose a secondary component that exhibits the opposite partitioning compared to component 1, but exhibits more partitioning compare to the other species. In our first analysis, we start with the solvent as this secondary dominant component. If this is the case, $y_1\rightarrow 1-\epsilon$, where $\epsilon$ is vanishingly small, with a solvent dominated dilute phase, meaning also $z\rightarrow 1$. This is equivalent to Flory's approximation in the single polymer case, and we can effectively solve the system as if no other polymers are present. In the limit of $\epsilon\rightarrow 0$, where correspondingly $w_i$ for $i>1$ go to zero, we get:
% \begin{equation}
%     h(z)\approx 1+{(h(y_1)-1)/N_1}
% \end{equation}
% which has solutions in terms of the inverse FH function:
% \begin{equation} \label{eq:eqAPPSolution}
%     z=h^{-1}\left(1+{(h(y_1)-1)/N_1}\right).
% \end{equation}
% We can subsequently solve for the set $y_i$ describing the partitioning of other polymers by applying equation \ref{eq:eqyidefined}. We can map this approximation to all of composition space for a specific value of $y_1$, $w_i$,  and then checking that the master equation is satisfied up to some tolerance to accept the approximation prediction, or to reject it.

% In many cases, though, the dilute phase in one polymer is the dense phase in the other, and vice versa, for a given polymer pair. In other words, the solvent may not be significantly partitioned between phases. If that is the case, we can seek approximations by assuming that one of the polymers is the ``solvent" while the other is the polymer, effectively rescaling the theory in these dominant composition coordinates. If we were to do this with component $j$ as the solvent, and component $y_i$ the dominant partitioning component, we would find:
% \begin{equation} %THIS HAS BEEN CHECKED
%     y_j=-h^{-1}\left(1+{(h(y_i)-1)N_j/N_i}\right).
% \end{equation}
% where $y_j$ is chosen to have the opposite sign of $y_i$. All other composite variables, $y_k$, can be computed by the analogue of equation \ref{eq:eqyidefined} that treats component $j$ as the ``solvent'' component that satisfies incompressibility, namely:
% \begin{equation} %CHECK THIS
%     y_k=\tanh\left(-\frac{N_k}{N_j}\left(\frac{\eta_k}{\eta_i}-1\right)\tanh^{-1}(y_j)+\frac{\eta_k N_k}{\eta_i N_i} \tanh^{-1}(y_i) \right)
% \end{equation}
% where for the solvent $y_0=-z$.


% We can use this procedure to map out the areas near the boundary of our composition space, where $y_1 \rightarrow 1$ or $w_iy_1\rightarrow \pm \infty$. Further, by considering each possible pair of polymers or solvent combination, we can generate a combinatoric set of approximations that span all regions far from the critical point, that may at least make for useful guesses for the full master equation. Similar to the one-polymer case, we expect that these approximations will be most accurate when there are significant differences in the polymer lengths.




% \section{Approximations near the critical point}
% Near the critical point, the partitioning of each species becomes negligible, i.e., $\mid y_i\mid, \mid z\mid \ll 1 $, and the master equation is:
% \begin{equation}\label{eq:eqCrit}
%     z^2=\frac{\sum_i w_i y_i^2/N_i}{\sum_i w_i}
% \end{equation}
% with the chemical potential constraint setting:
% \begin{equation}
%     y_i=N_i(\eta_i-1)z+\eta_i \frac{N_i}{N_1} y_1
% \end{equation}
% This approximation is valid as long as:
% \begin{equation}
% \begin{split}
%         &z\ll 1 \quad \& \quad z\ll \frac{1}{N_i(\eta_i-1)} \\
%         &y_1\ll 1 \quad \& \quad y_1\ll \frac{N_1}{N_i\eta_i}
% \end{split}
% \end{equation}
%  Combined, these equations give a quadratic equation for $z$ which can be solved exactly. The quadratic equation explicitly is: 
% \begin{equation}
% \begin{split}
%         0=&z^2\left(-1+\frac{\sum_i w_i N_i(\eta_i-1)^2}{\sum_i w_i}\right)\\
%         &+z\left(\frac{\sum_i 2w_i N_i\eta_i(\eta_i-1)y_1/N_1}{\sum_i w_i}\right)\\
%         &+\frac{\sum_i w_i N_i\eta_i^2y_1^2/N_1^2}{\sum_i w_i}.
% \end{split}
% \end{equation}
% Picking the set $w_i$ and $y_1$, we solve for $z$, picking the root that gives positive $\beta_i$ for all $i$, if in fact either root gives positive $\beta_i$.



% % For the multicomponent case, a lot of complexity is removed if we can assume something about the value of $x$, corresponding to limiting values of $z$, bounded by -1 and 1. The limits of $z$ correspond to the relative difference in solvent content between phases. If $z$ goes to $0$, corresponding to small differences in solvent content between the phases, the value of $x=\tanh^{-1}(z)$   goes to 0. Along with $w_1=1$, the system of equations for $w_i$ becomes:
% % \begin{equation}
% %     \sum_j \left[\frac{x_i}{N_i}\alpha_{1j} -\frac{x_1}{N_1}\alpha_{ij}\right]w_j=0
% % \end{equation}
% % This can easily be inverted to get $w_i$ explicitly, with all variables known. 

% % In the limit $z=\pm 1$, the solvent content is very different between the phases, and $x\rightarrow \pm \infty$. If this is the case, then the equations for $w_i$ becomes:
% % \begin{equation}
% %     \sum_j \left[\left(\alpha_{1j}-\alpha_{ij}\right)\right]w_j=0
% % \end{equation}
% % which is again invertible easily, as long as the matrix is not singular.

% % Equipped with all the values of $w_j$, one can determine $\mathbf{\phi}_A$ and $\mathbf{\phi}_B$, then check the value of $z$ to verify if the approximation is decent or not.

% % \subsubsection{Polydisperse polymer of one type}
% % In this case, we can again get great simplification if $z\rightarrow 0$ or $z\rightarrow \pm 1$.

% \section{Adding non-interacting ``crowders''}
% To add to our list of analytical solutions, we can consider the case of non-interacting  crowders added to a strongly interacting polymer in solvent. Although this ideal non-interacting assumption may be rare in reality, it may be a reasonable approximation if one polymer self-interaction is much larger in magnitude than all other interactions. We assume that the dominant polymer is $i=1$, where $\alpha_{11}=1$.  However, if non-interacting crowders are added with species index: $2<i<M$, then since their corresponding rows and columns $\alpha_{ij}=0$, we have $\eta_i=0$ for these species. Therefore, the $\alpha$ matrix only has one entry.   

% For the non-interacting polymers, we have:
% \begin{equation}
%     y_i=\tanh\left(-N_i\tanh^{-1}(z)\right).
% \end{equation}

% The master equation can be written as:
% \begin{equation}
%     \begin{split}
%         \frac{x}{z}=&1+\frac{\left(h(y_1)-1\right)/N_1}{\sum_i w_i}\\
%         &+\frac{\sum_{i=2}^{M} w_i\left(-\frac{N_i x}{\tanh\left(-N_i\tanh^{-1}(z)\right)}-1\right)/N_i}{\sum_i w_i}
%     \end{split}
% \end{equation}

% If this is the case, then we can again solve the equation for $z$ explicitly with the inverse FH function $h^{-1}$, exactly as we did for the one component case:


% \section{Extensions to other equations of state}
% Here, we can explore how this formulation could be extended to other equations of state based on a lattice, focusing only on the polymer-solvent system. In other theories, one could replace the $-\chi \phi^2$ term in the free energy density by:
% \begin{equation}
%     -\chi \tilde{f}_\mathrm{int}(\phi)
% \end{equation}
% which is equivalent to assuming a $\phi$-dependent $\chi$ parameter.

% In this case, from the chemical potential, we arrive at:
% \begin{equation}
%     \chi=\frac{\frac{2}{N}\tanh^{-1}(y)+2\tanh^{-1}(z)}{\tilde{f}_\mathrm{int}^{\prime}(\phi_A)-\tilde{f}_\mathrm{int}^{\prime}(\phi_B)}
% \end{equation}
% And from the pressure, we have:
% \begin{equation}
%     \chi=\frac{\left(\frac{1}{N}-1\right)(\phi_A+\phi_B) y+2\tanh^{-1}(z)}{\tilde{f}_\mathrm{int}(\phi_B)-\tilde{f}_\mathrm{int}(\phi_A)+\phi_A\tilde{f}_\mathrm{int}^{\prime}(\phi_A)-\phi_B\tilde{f}_\mathrm{int}^{\prime}(\phi_B)}
% \end{equation}

% Substituting in:
% \begin{equation}
%     \begin{split}
%         &\phi_A=\frac{z(1+y)}{z+y}\\
%         &\phi_B=\frac{z(1-y)}{z+y}
%     \end{split}
% \end{equation}
% and equating the values of $\chi$, we generally have a nonlinear equation for one unknown ($z$) in terms of one specified variable ($y$)---reducing our system of two equations down to one equation. While not guaranteed, one may be able to decouple the $z$ and $y$ dependence, defining a function similar to the FH function $h()$ for a given functional interaction form.



% While this procedure is marginally better than solving the full system of two equations for the polymer-solvent system, it can be especially helpful for the multicomponent case. There, we can reduce down large systems of coupled equations into one nonlinear equation that gives us an implicit solution to $\chi$. We leave these generalizations to future work.

% % \subsection{Decoupling of Equations}
% % Subtracting the second chemical equilibrium equation from the first in equation \ref{eq:eqChemEq}, we have:
% % \begin{equation}
% %     \frac{1}{N}\ln\left(\frac{\phi_1}{\phi_B}\right)-\left(\frac{1}{N}-1+2\chi\right) (\phi_1-\phi_B)+\chi(\phi_1^2-\phi_B^2)=0
% % \end{equation}
% % Next we define auxiliary variables $A$ and $B$:
% % \begin{equation}\label{eq:defAB}
% %     \begin{split}
% %         &A=\phi_1-\phi_B\\
% %         &B=\phi_1+\phi_B
% %     \end{split}
% % \end{equation}
% % and plug in to get:
% % \begin{equation}\label{eq:eqIntermediate}
% %     \frac{1}{N}\ln\left(\frac{A+B}{B-A}\right)-\left(\frac{1}{N}-1+2\chi\right) A+\chi AB=0
% % \end{equation}
% % If we define $y$ as:
% % \begin{equation}\label{eq:defy}
% %     y=\frac{A}{B}=\frac{\phi_1-\phi_B}{\phi_1+\phi_B}
% % \end{equation}
% % , we can rewrite equation \ref{eq:eqIntermediate} as:
% %     \begin{equation}
% %     \ln\left(\frac{1+y}{1-y}\right)-\left(1-N+2N\chi\right) By+N\chi B^2y=0.
% % \end{equation}
% % Next, noticing the quadratic form in $B$, we can explicitly solve for $B$ in terms of $y$:
% % \begin{equation}\label{eq:eqBW_general}
% % B=\beta+\beta\sqrt{1-w}
% % \end{equation}
% % with
% % \begin{equation}\label{eq:eqWY_general}
% %     \begin{split}
% %         &\beta=1+\frac{1}{2N\chi}-\frac{1}{2\chi}\\
% %         &w=\frac{1}{N\chi \beta^2 y}\ln\left(\frac{1+y}{1-y}\right)
% %     \end{split}
% % \end{equation}


% % Next, with an explicit solution for $B$ in terms of y, we can now substitute in for $B$ to eliminate one unknown, so that we have one master equation that is in terms of $y$. We can either implement this substitution in the chemical potential equation or the pressure equation in \ref{eq:eqChemEq}, to get $g_1(y)=0$ or $g_2(y)=0$ respectively. First, for the chemical potential equilibrium equation, we express it in terms of $A$ and $B$:
% % \begin{equation}
% % \frac{1}{N}\ln\left(\frac{A+B}{B-A}\right)-\ln\left(\frac{2-(A+B)}{2-(B-A)}\right)-2\chi A=0
% % \end{equation}
% % Or in terms of $y$:
% % \begin{equation}
% %     \chi \beta^2 y w-\ln\left(\frac{2-B(1+y)}{2-B(1-y)}\right)-2\chi By=0
% % \end{equation}
% % If we plug in the relationships for $B$ and $w$ in terms of $y$ from equations \ref{eq:eqBW_general} and \ref{eq:eqWY_general}, the above equation is the master equation for $g_1(y)=0$.

% % We could also write the master equation equivalently by substituting directly for the pressure. Here we have:
% % \begin{equation}
% %     \left(\frac{1}{N}-1\right)yB-\ln\left(\frac{2-B(1+y)}{2-B(1-y)}\right)-\chi B^2 y=0
% % \end{equation}

% % The master equation is transcendental, and there is no clear way to solve it exactly. Therefore, while we cannot arrive at a purely analytical solution, we have reduced the system of equations into one equation with one variable, $y$.

% % What is the use of such an equation? First, it can be solved numerically with more ease than the coupled system. Secondly, it can be a useful reference point from which to derive analytical approximations, where we directly expand at specific values of $y$, rather than having to make simultaneous approximations for $\phi_1$ and $\phi_B$. We explore this strategy in the following sections.

% % \subsection{Limit 1: $\epsilon=1-y \ll 1$, away from the critical point}
% % % The master equation $g_1$ becomes:
% % % \begin{equation}
% % %     \chi \beta^2 w-\ln(1-B)-2\chi B=0
% % % \end{equation}
% % The first limit is $\epsilon=1-y \ll 1$. We subsitute into the master equation, and drop all terms proportional to $\epsilon$. After this procedure, the master equation for $g_2$ becomes:
% % \begin{equation} \label{eq:eqMaster}
% %     \left(\frac{1}{N}-1\right)B-\ln(1-B)-\chi B^2=0
% % \end{equation}
% % which is equivalent to $g_1$. The master equation essentially states that the dilute phase pressure goes to zero, which must be matched by the dense phase, which dominates in its contribution to $B$. We can solve the equation for $B$, then use the value of $B$ to find $w$, then use $w$ to get $y$. 

% % The relationship between $B$ and $w$ follows directly from equation \ref{eq:eqBW_general}:
% % \begin{equation}\label{eq:eqwb2}
% %     w=1-\left(\frac{B}{\beta}-1\right)^2.
% % \end{equation}
% % Also, we have from the definition of $w$, for $\epsilon \ll 1$:
% % \begin{equation}\label{eq:eqWEps}
% %     w=-\frac{1}{N\chi\beta^2}\ln(\epsilon/2)
% % \end{equation}
% % or 
% % \begin{equation}\label{eq:eqyw}
% %     y=1-\epsilon=1-2\exp(-N\chi\beta^2 w).
% % \end{equation}

% % If equation \ref{eq:eqMaster} is solved exactly for $B$ and then equations \ref{eq:eqwb2} and \ref{eq:eqyw} are used to determine $y$, then the solution is asymptotically exact for large $\chi$. But $\chi$ does not have to be exceedingly large for the approximation to work, especially for large $N$. For example, a 5\% error in dilute phase concentration is predicted at $\chi=0.64$ for $N=200$, just a small distance from the critical point defined by $\chi_c=0.57$. And the relative error only becomes better for larger values of $\chi$. 


% % It would be most helpful, then, if we could directly solve or approximate master equation \ref{eq:eqMaster} explicitly in terms of $B$. However, note that equation \ref{eq:eqMaster} contains three terms that are all generally important when $N\neq 1$, even in the limit $\epsilon\ll 1$. Unfortunately, even this simplified equation has solutions that can only be expressed in terms of generalized Lambert-W functions \cite{mugnaini2014generalization} which are not readily available in most scientific computing packages. The analytical solution to equation \ref{eq:eqMaster} in terms of a general series is derived in Appendix A, though it may be difficult to evaluate to sufficient accuracy  or extract intuition from such a series.

% % So given these complications, how can we approximate the solution to equation \ref{eq:eqMaster} in terms of simple functions? Since the solution can exhibit values of $B$ close to 1, the strong nonlinearity in the $\ln$ term must be maintained.  Even so, we can get a decent approximate solution by linearizing the quadratic term around a specific value of $B$, $B_0$:
% % \begin{equation}
% %     B^2\approx B_0^2+2B_0(B-B_0),
% % \end{equation}
% % or substituting in this expression into equation \ref{eq:eqMaster}:
% % \begin{equation}
% %     \left(\frac{1}{N}-1\right)B-\ln(1-B)-\chi B_0^2-2\chi B_0(B-B_0)=0.
% % \end{equation}
% % Substitution of $1/N$ in terms of $\beta$ gives:
% % \begin{equation}
% %     2\chi(\beta-1)B-\ln(1-B)+\chi B_0^2-2\chi B_0B=0,
% % \end{equation}
% % and choosing $B_0=\beta$ gives:
% % \begin{equation}
% %     -2\chi B-\ln(1-B)+\chi \beta^2=0.
% % \end{equation}
% %  The choice of $B=\beta$ is reasonable because it is the minimum bound for $B$ via equation \ref{eq:eqBW_general}, though a more informed prediction could improve the accuracy of the approximation.
 
% % The solution to the above equation is:
% % \begin{equation} \label{eq:eqhighchi}
% %     B=1+\frac{\mathrm{W}\left(-2\chi e^{\beta^2\chi-2\chi}\right)}{2\chi}, \quad N>1
% % \end{equation}
% % where $\mathrm{W}()$ is the Lambert-W function.


% % Note that some error is incurred when approximating the solution to equation \ref{eq:eqMaster} through this process, and even some systematic error persists in the asymptotic limit of $\epsilon\ll1$. Improvements can be made by providing a better guess for $B_0$, such as $B_0=\beta(1+1/(2\chi+1))$ (empirically determined). If we wish for asymptotically exact results, we can solve equation \ref{eq:eqMaster} either numerically or evaluating its series solution without much trouble---significantly simpler than solving the coupled system of equations.

% % Despite these shortcomings, these approximations are all superior to those previously made at large $\chi$ \cite{doi2013soft, qian2022analytical}, where
% % \begin{equation}
% % \begin{split}
% %         &\phi_1=1-e^{-(\chi+1)}\\
% %         &\phi_B=e^{-N(\chi-1)}
% % \end{split}
% % \end{equation} 
% % which would mean:
% % \begin{equation}
% % \begin{split}
% %         y&\approx(1-e^{-(\chi+1)}-e^{-N(\chi-1)})(1+e^{-(\chi+1)}-e^{-N(\chi-1)})\\
% %       &y\approx 1-2e^{-N(\chi-1)}
% % \end{split}
% % \end{equation}
% % These exponential scalings are only valid with $\chi\gg 1$ and $N\gg1$, where:
% % \begin{equation}
% %     -N\chi\beta^2\approx -N(\chi-1)
% % \end{equation}
% % and $B=\beta$, or equivalently, $w=1$.



% % \subsection{Limit 2: $\epsilon=y \ll 1$, Near the critical point}
% % The second limit is $\epsilon=y \ll 1$, which is valid only near the critical point.

% % In this limit, we can expand the master equation in $y$. At leading order, we have:
% % \begin{equation}
% % \alpha_3 y^3+\alpha_5y^5+\alpha_7 y^7+\dots=0.
% % \end{equation}
% % We do not explicitly include the expressions for any $\alpha$ values due to their algebraic complexity, but they can be evaluated explicitly in terms of $N$ and $\chi$. 

% % Since $y=0$ is not a valid solution away from the critical point, to leading order, we have:
% % \begin{equation}\label{eq:eqSmall_2terms}
% %     y=\sqrt{-\alpha_3/\alpha_5}
% % \end{equation}
% % where we have chosen the positive root. 

% % Since these approximations are only valid near the critical point, we can also expand in $\chi-\chi_c$ to get simpler closed form solutions. In this case, we can solve the coupled equations directly \cite{qian2022analytical} to arrive at:
% % \begin{equation}\label{eq:eqSmall_2terms_critical}
% %     y=\frac{\sqrt{3(\chi-\chi_c)/(2\chi_c^2\sqrt{N})}}{\phi_c}, 
% % \end{equation}
% % with critical volume fraction defined as:
% % \begin{equation}
% %     \phi_c=\frac{1}{1+\sqrt{N}}.
% % \end{equation}


% % If we wish for even more accuracy compared to equations \ref{eq:eqSmall_2terms} and \ref{eq:eqSmall_2terms_critical}, we can include all three terms to evaluate $y$:
% % \begin{equation}\label{eq:eqysmall_multiple_terms}
% %     y=\sqrt{\frac{-\alpha_5-\sqrt{\alpha_5^2-4\alpha_7\alpha_3}}{2\alpha_7}}
% % \end{equation}



% % Note however that these approximations are not too accurate unless $y$ is very small due to the strong nonlinear (singular) response of the master equation. Therefore, we will focus on the predictions of Limit 1, and extend it to be uniformly valid near the critical point.
% % In this limit, we can relate $B$ and $y$ as:
% % \begin{equation}
% % \begin{split}
% %         &B=\beta+\beta\sqrt{1-\frac{2}{N\chi\beta^2}}-\frac{\beta y^2}{3 N\chi \beta^2\sqrt{1-\frac{2}{N\chi\beta^2}}} \\
% %         &B=\alpha_0+\alpha_2 y^2
% % \end{split}
% % \end{equation}
% % where we use the shorthand $\alpha_0$ and $\alpha_2$ to write the expressions more compactly.


% % In the limit of $y\ll 1$, the master equation becomes:
% % \begin{equation}
% %         B y\left(B\left(\frac{1}{2-B}-\chi\right)+\frac{1}{N}\right)+\frac{2 B^3 y^3}{3(2-B)^3}+\dots=0
% % \end{equation}
% % which has a leading order solution of $y=0$. With $y=0$, we have:
% % \begin{equation}
% %     B=\beta+\beta\sqrt{1-\frac{2}{N\chi\beta^2}}
% % \end{equation}

% % If we retain terms up to $y^3$, we get:

% % \begin{equation}\label{eq:eqysmall}
% % \begin{split}
% %      &\alpha_0 y\left((\alpha_0+\alpha_2y^2)\left(\frac{1}{2-\alpha_0}-\chi\right)+\frac{1}{N}+\frac{\alpha_2 y^2}{(2-\alpha_0)^2}\right)\\
% %      &+\alpha_2 y^3\left(\alpha_0\left(\frac{1}{2-\alpha_0}-\chi\right)+\frac{1}{N}\right)+\frac{2\alpha_0^3 y^3}{3(2-\alpha_0)^3}=0
% % \end{split}
% % \end{equation}

% % Factoring out a factor of $y$, we are left with a quadratic equation for $y$, which can be written as:
% % \begin{equation}
% %     \gamma_0+\gamma_2y^2=0
% % \end{equation}
% % (we do not include the detailed expression due to its algebraic complexity). The solution is given by $y=\sqrt{-\gamma_0/\gamma_2}$. We choose the positive root such that $y>0$.


% % \subsection{Uniform solution}
% % Here, we will attempt to extend the validity of the approximate solution to Limit 1 $(\epsilon=1-y\ll1)$ to make it work also near the critical point. The prediction for $B$ in equation \ref{eq:eqhighchi} becomes complex valued when:
% % \begin{equation}
% %     -2\chi e^{\beta^2\chi-2\chi}<-\frac{1}{e}.
% % \end{equation}
% % Here, we will adopt the real part of that expression, such that:
% % \begin{equation} \label{eq:eqhighchi_real}
% %     B=1+\frac{\mathrm{Re}\left(\mathrm{W}\left(-2\chi e^{\beta^2\chi-2\chi}\right)\right)}{2\chi}.
% % \end{equation}

% % Here, for completeness in this section, we repeat the relationship between $w$ and $B$, which follows directly from equation \ref{eq:eqBW_general}:
% % \begin{equation}\label{eq:eqwb_real}
% %     w=1-\left(\frac{B}{\beta}-1\right)^2.
% % \end{equation}
% % and the definition of $\beta$ is:
% % \begin{equation}
% %     \beta=1+\frac{1}{2 N\chi}-\frac{1}{2\chi}
% % \end{equation}

% % Next, near the critical point, the value of $w$ approaches $w=2/(N\chi\beta^2)$ as $\epsilon\rightarrow 1$, which is not captured with our asymptotic expression valid for $\epsilon\rightarrow 0$. In order to reproduce the limits as $\epsilon\rightarrow 1$ and maintain the behavior as $\epsilon\rightarrow 0$, we empirically assume that:
% % \begin{equation}
% %     w=-\frac{1}{N\chi\beta^2}\left[\ln(\epsilon/2)+\epsilon(-\ln(1/2)+2)\right]
% % \end{equation}
% % which can be solved for $\epsilon$:
% % \begin{equation}\label{eq:eqyw_extended}
% %     y=1-\epsilon=1-\frac{\mathrm{W}\left([2\ln(2)-4]\exp(-N\chi\beta^2 w)\right)}{2-\ln(2)}.
% % \end{equation}
% % In order to find the dilute and concentrated phase concentrations, we can simply apply the definitions of $B$ and $y$ in equations \ref{eq:defAB} and \ref{eq:defy} explicitly.


% % % The simplest criterion for switching between the two limits can be based on the physical boundaries imposed on the variable $y$. $y$ must be real and less than 1. Note that equation \ref{eq:eqhighchi} becomes complex valued when:
% % % \begin{equation}
% % %     -2\chi e^{\beta^2\chi-2\chi}<-\frac{1}{e}.
% % % \end{equation}
% % % This sets a natural boundary on the validity of the approximations,demarcating the application of each approximation.
% % \section{Results}
% % \subsection{Comparison of approximation predictions to numerics}

% % First, we can demonstrate the accuracy of the prediction on a phase diagram. The uniform solution derived from limit 1 seem to work especially well far from the critical point, and can work well near the critical point when $N$ is large. The extension to the critical point introduces artificial cusps in the approximate prediction, which are very apparent for the concentrated phase volume fractions on a linear scale plot.

% % Next, for a range of $N$ and $\chi$ values, we solve to get the value of $y$ numerically. Then, we compare to the prediction (from Limit 1) made by applying equations \ref{eq:eqhighchi_real}, \ref{eq:eqwb_real}, and \ref{eq:eqyw_extended}, in that order, to arrive at $y_\mathrm{pred}$.  For now, we do not analyze the accuracy of equations \ref{eq:eqSmall_2terms_critical} or \ref{eq:eqysmall_multiple_terms} (Limit 2) because they tends to break down very quickly, especially on the practically relevant log-scale.

% % To start, we plot a surface of the $y$ (Fig. 3) and $\ln(1-y)$ (Fig. 4). Note that the black lines correspond to the critical $\chi$ value at each value of $N$. 

% % % There is white space in the $y_\mathrm{pred}$ plots because the prediction returns a complex value at those locations, due to the argument of the Lambert-W function. 

% % Next, we can analyze the error for $y$, $\ln(1-y)$, and $1-y$. We define the error as:
% % \begin{equation}
% %     \mathrm{Error}=\mid\frac{y-y_\mathrm{pred}}{y}\mid
% % \end{equation}
% % We see that the errors are quite small over the range of valid $N$ and $\chi$ values for the prediction, especially for $y$ and $\ln(1-y)$. For accurate prediction of a phase diagram, we ultimately are looking for accurate $\ln(1-y)$ or $1-y$.



% % \subsection{Fitting to experimental data}
% % \appendix
% % \section{Series solution to approximated master equation}
% % Here, we derive an analytical solution to the approximated master equation, equation \ref{eq:eqMaster}. First, we recast the equation in the form\cite{mugnaini2014generalization}:
% % \begin{equation}\label{eq:eq_transformed}
% %     z=a+le^{-z^2/2}
% % \end{equation}
% % Which is achieved with definitions:
% % \begin{equation}
% %     \begin{split}
% %         &z=\sqrt{2\chi}B-\frac{1}{\sqrt{2\chi}}\left(\frac{1}{N}-1\right)\\
% %         &a=\sqrt{2\chi}-\frac{1}{\sqrt{2\chi}}\left(\frac{1}{N}-1\right)\\
% %         &l=-\sqrt{2\chi}e^{\frac{1}{4\chi}\left(\frac{1}{N}-1\right)^2}.
% %     \end{split}
% % \end{equation}
% % The solution to the above equation can be written in terms of the Lagrange reversion formula:
% % \begin{equation}
% %     z=a+\sum_{n=1}^\infty \frac{l^n}{n!}\left[\left(\frac{\mathrm{d}}{\mathrm{d}z} \right)^{n-1} e^{-nz^2/2}\right]_{z=a}
% % \end{equation}
% % Using the property of (probabilistic) Hermite polynomials:
% % \begin{equation}
% %     \mathrm{He}_n(z)=(-1)^n e^{z^2/2}\left(\frac{\mathrm{d}}{\mathrm{d}z} \right)^{n} e^{-x^2/2},
% % \end{equation}
% % we can therefore rewrite the coefficients of the series either in terms of probabilistic Hermite polynomials, $\mathrm{He}$,  or physics Hermite polynomials, $\mathrm{H}$, which differ by a recursive factor:
% % \begin{equation}
% % \begin{split}
% %     &z_n(a)=\left[\left(\frac{\mathrm{d}}{\mathrm{d}z} \right)^{n-1}  e^{-nz^2/2}\right ]_{z=a}\\ 
% %     &=(-1)^{1-n} n^{(n-1)/2} e^{-n a^2/2} \mathrm{He}_{n-1}(\sqrt{n}a)\\
% %     &=(-1)^{1-n} \left(\frac{n}{2}\right)^{(n-1)/2} e^{-n a^2/2} \mathrm{H}_{n-1}\left(\sqrt{\frac{n}{2}}a\right)\\
% % \end{split}
% % \end{equation}
% % In order to evaluate the series accurately, we typically need the number of terms in the series that exceeds the value $N$. However, at large values of $n>100$, it is difficult to maintain numerical accuracy. Therefore, the analytical solution is of limited use without modification or asymptotic expressions for the terms in the series as $n\rightarrow\infty$. 

% % For better convergence, we can recenter the series such that the first term gives $B=\beta$, which is a better bound for $B$ than $B=1$. We use the following identity:
% % \begin{equation}
% %     \gamma=(a-a_0)-l_0 e^{(a-a_0)^2/2}+l_0 e^{-\gamma^2/2}
% % \end{equation}
% % where clearly $\gamma=a-a_0$, can identically be expressed as a solution to equation \ref{eq:eq_transformed}.
% % \begin{equation}
% % \begin{split}
% %         &\gamma=\alpha+\sum_{n=1}^\infty \frac{l_0^n}{n !} \gamma_n(\alpha) \\
% %         &\alpha=(a-a_0)-l_0 e^{(a-a_0)^2/2}.
% % \end{split}
% % \end{equation}
% % where $\gamma_n(\alpha)$ has the same functional form as $z_n(a)$. From here, we choose $a_0$ to give $z$ at $B=\beta$ as a first term:
% % \begin{equation}
% %     a-l_0 e^{-(a-a_0)^2/2}=\beta\sqrt{2\chi}-\frac{1}{\sqrt{2\chi}}\left(\frac{1}{N}-1\right)
% % \end{equation}
% % which is satisfied by:
% % \begin{equation}
% %     a_0=a\pm \sqrt{\ln\left(\frac{l_0^2}{2\chi(1-\beta)^2}\right)}.
% % \end{equation}

% % Therefore, we can rewrite the solution for $z$ as:
% % \begin{equation}
% %     z=a-l_0 e^{-(a-a_0)^2/2}+\sum_{n=1}^\infty \frac{l^n}{n !} z_n(\alpha)+\frac{l_0^n}{n !} \gamma_n(\alpha)
% % \end{equation}
% % Note that the value of $l_0$ is not specified, but is constrained to be $l_0\geq \sqrt{2\chi}(1-\beta)$. Therefore, it can be chosen to improve convergence of the series or numerical accuracy of individual terms in the series.

% % Using the above fist two terms before the summation, we get $B=\beta$. Following terms give corrections to this approximation, and therefore fewer terms are needed since $B$ is typically close to $\beta$. 


% % \begin{figure}[t!]
% % \centerline{\includegraphics[scale=0.6]{phase_diagram_log.pdf}}
% % \caption{Phase diagram for $N=10, 50, 100, 500$. Blue lines are the approximation and black lines are the numerical result. }
% % \end{figure}

% % \begin{figure}[t!]
% % \centerline{\includegraphics[scale=0.6]{phase_diagram_linear.pdf}}
% % \caption{Phase diagram for $N=10, 50, 100, 500$. Blue lines are the approximation and black lines are the numerical result. }
% % \end{figure}
% % \begin{figure}[htbp!]
% % \centerline{\includegraphics[scale=0.6]{linear_plot.pdf}}
% % \caption{Value of y and $y_\mathrm{pred}$ varying $N$ and $\chi$}
% % \end{figure}

% % \begin{figure}[t!]
% % \centerline{\includegraphics[scale=0.6]{log_plot.pdf}}
% % \caption{Value of $\ln(1-y)$ and $\ln(1-y_\mathrm{pred})$ for varying $N$ and $\chi$}
% % \end{figure}

% % \begin{figure}[t!]
% % \centerline{\includegraphics[scale=0.6]{error_linear.pdf}}
% % \caption{Figure : Error of y and $y_\mathrm{pred}$ for varying $N$ and $\chi$}
% % \end{figure}

% % \begin{figure}[t!]
% % \centerline{\includegraphics[scale=0.6]{error_log.pdf}}
% % \caption{Error of $\ln(1-y)$ and $\ln(1-y_\mathrm{pred})$ for varying $N$ and $\chi$}
% % \end{figure}


% % \begin{figure}[t!]
% % \centerline{\includegraphics[scale=0.6]{error_minus.pdf}}
% % \caption{Error between $(1-y)$ and $(1-y_\mathrm{pred})$ for varying $N$ and $\chi$}
% % \end{figure}




% % Solving for $w$ in terms of $B$, we have:
% % \begin{equation}
% %     w=1-\left(\frac{B}{\beta}-1\right)^2=-\frac{B^2}{\beta^2}+2\frac{B}{\beta}
% % \end{equation}
% % We can therefore rewrite the equation for $g_1$ as:
% % \begin{equation}
% %     -\chi B^2+2\chi B \beta-\ln(1-B)-2\chi B=0
% % \end{equation}

% % \begin{equation}
% %     -\chi B^2+ B (\frac{1}{N}-1)-\ln(1-B)=0
% % \end{equation}

    



% % The critical point, where $f^{\prime\prime\prime}(\phi)=0$:
% % \begin{equation}
% %     \phi_c=\frac{1}{1+\sqrt{N}}, \quad \chi_c=\frac{1}{2}\left(1+\frac{1}{\sqrt{N}}\right)^2
% % \end{equation}

% % Expanded around the critical point, $\delta\phi=\phi-\phi_c$ and neglecting terms that are constant or linear in $\phi$:
% % \begin{equation}
% %     \tilde{f}\approx (\chi-\chi_c)\delta\phi^2+\frac{\chi_c^2\sqrt{N}}{3}\delta\phi^4+\frac{\ell^2}{2}{\delta\phi^\prime}^2
% % \end{equation}


% % Here, we derive a minimal model of electrolyte phase separation as a salt approaches its solubility limit in water.  We demonstrate the relationship between the phase boundary, the distance from the spinodal curve, and the far-field decay of density from an interface.
















% \bibliography{library.bib}

% \end{document}

